Slice Sampling for General Completely Random Measures

Completely random measures provide a principled approach to creating flexible unsupervised models, where the number of latent features is infinite and the number of features that influence the data grows with the size of the data set. Due to the infinity the latent features, posterior inference requires either marginalization---resulting in dependence structures that prevent efficient computation via parallelization and conjugacy---or finite truncation, which arbitrarily limits the flexibility of the model. In this paper we present a novel Markov chain Monte Carlo algorithm for posterior inference that adaptively sets the truncation level using auxiliary slice variables, enabling efficient, parallelized computation without sacrificing flexibility. In contrast to past work that achieved this on a model-by-model basis, we provide a general recipe that is applicable to the broad class of completely random measure-based priors. The efficacy of the proposed algorithm is evaluated on several popular nonparametric models, demonstrating a higher effective sample size per second compared to algorithms using marginalization as well as a higher predictive performance compared to models employing fixed truncations.

==> algorithm.tex <==
\section{Slice Sampling Algorithm}

 Along with the auxiliary variables, we can then design a Gibbs sampler \cite{tierney94} that only condition on instantiated variables. Here we use a sampling strategy similar to \cite{teh07}. For atoms that are occupied, that is, for $1\le k<K^\star$ the algorithm samples: 
\[
	(V_k,\Gamma_k)|V_{1:\infty\backslash\{k\}},\Gamma_{1:\infty\backslash\{k\}}\eqd(V_k,\Gamma_k)|\Gamma_{k+1},\Gamma_{k-1}
\]
The equal in distribution is obtained by Markov property and independence of random perturbations.

 To sample $k\ge K^\star$ and beyond, we block-sample joint distribution of $(V_{K^\star:\infty},\Gamma_{K^\star:\infty})$ by progressively drawing from:
\[
	\left(V_k,\Gamma_k\right)|V_{1:k-1},\Gamma_{1:k-1}\eqd(V_k,\Gamma_k)|\Gamma_{k-1}
\]  
where the equal in distribution is obtained by Markov property. 

 This step terminates when $k=K$ since $x_{nk}=0$ almost surely for $k>K$. To show correctness, we can imagine the hypothetical ``algorithm'' re-instantiates the remaining weights from $K+1$ up to $\infty$ but are then re-written by future iterations, if any. The proof is in the appendix. Since we want to initialize as few variables as possible, the variables are drawn in reversed topological order of the graphical model as follows:

\begin{enumerate}[leftmargin=0.5cm]
	\item Draw independent $U_n\dist\distUnif\left[0,\xi(k_n^\star)\right]$ and decide truncation level $K$. This restricts the maximum number of features that we will need for the Gibbs sampler to proceed. In our experiment we used $\xi\left(k\right)=\exp\left(-\frac{k}{\sigma}\right)$ and tunned $\sigma$ by selecting the one with the highest effective sample size. It turns out $\sigma=0.7$ has always been optimal in all experiments, and very robust to different models and models of different dimensions. We also compared this with drawing auxiliary indices from $U_n\dist\distUnif\left(k_n^\star:2k_n^\star\right)$. Although this that does not need tuning like the deterministic sequence, it is comparatively less efficient in most cases. To manage memory allocation in varying dimensions, we recommend amortized resizing of dynamic array $x$ or use coordinate form sparse matrix to reduce storage cost. 
	\item Sample latent combinatorial variable $x_{nk}$ from:
	\[
		\Pr\left(x_{nk}=r|\tre\right)&\propto f\left(y_n|x_n,\psi\right)h\left(x_{nk}|\tau\left(V_k,\Gamma_k\right)\right)\cr
		&\distUnif\left[0\le U_n\le\xi\left(k_n^\star\left(x_{nk}=r\right)\right)\right]
	\]
	where $k_n^\star\left(k\right)$ is the last occupied feature for data $n$ after resetting the entry $k$. That is, if $x_{nk}$ for $k>k_n^\star$ takes a positive value that was previously zero, then the last occupied index should reset to the new $k$; if $k>k_n^\star$ sets a oreviously positive value to zero, then $k_n^\star$ should be reset to the previously second last occupied index. Let $k_n^\star$ be the last occupied indicies before the update and $k_n^{\star\star}$ be the second last occupied indicies before the update, then:
	\[
		k_n^\star\left(x_{nk}=r\right)=\begin{cases}
		k_n^{\star\star}&k=k_n^\star,r=0\cr
		k&k>k_n^\star,r>0\cr
		k_n^\star&\text{ otherwise}
		\end{cases}
	\]
	Since we're conditional on slice variable $U_n$, we only need to sample up to $K$ because every $x_{nk}\eqas0$ for $k\ge K$. This step can be made parallel or vectorized across $N$ data points and the likelihood can be updated recursively across $K$ features. We cannot make it this step parallel across $K$ because of the dependencies through $k_n^\star$. In many instances, one can devise lazy-update rule to recursively compute the likelihood, since at each $k$ only a subset of the $x_{nk}$'s are modified. Once $x_{nk}$'s are updated, it is necessary to update $k_n^\star$ accordingly and it's often helpful to update sufficient statistic $\sum_{n=1}^Nx_{nk}$ for latter calculation.  
	\item Sample latent features $\psi$ from:
	\[
		p\left(\psi|\tre\right)&\propto\left(\prod_{n=1}^Nf\left(y_n|x_n,\psi\right)\right)H\left(\psi\right)
	\]
	using either conjugacy between $f$ and base measure $H$ or Metropolis within Gibbs. We do not integrate out latent features because otherwise $x_{nk}$'s will be coupled across $N$, thus the inference on this graph will not be  parallelizable. If the matrix-valued posterior is well-understood then one can aim to sample $\psi$ as a whole instead of sampling from $p(\psi_k|\tre)$. 
	\item If $K^\star>0$, then update the instantiated sticks $\left(V_k,\Gamma_k\right)$ conditional on the nearest sticks for $k=1,\cdots,K^\star-1$ from:
	\[
		p\left(V_k,\Gamma_k|\tre\right)&\propto\left(\prod_{n=1}^Nh(x_{nk}|\tau(V_k,\Gamma_k))\right)g(V_k)\cr
		&\distUnif\left[\Gamma_{k-1}\le\Gamma_k\le\Gamma_{k+1}\right]
	\]
	We can only sample up to $K^\star-1$ because features starting $K^\star$ might not have been instantiated previously. We do not sample up to $K^\star-1$ because we don't want the order of Markov kernel composition to on the states and it's easy to show that the resulting chain has the posterior as the stationary distribution using the result by \cite{tierney94}. 
	
	\item Udpate the remaining sticks $\left(V_k,\Gamma_k\right)$ for $k=K^\star,\cdots,\infty$ conditional only on the previous sticks from:
	\[
		&p\left(V_k,\Gamma_k|V_{1:k-1},\Gamma_{1:k-1},\tre\right)\cr
		&\propto\Pr\left(x_{1:N,k+1:\infty}=0|\Gamma_k\right)\left(\prod_{n=1}^Nh\left(x_{nk}|\tau(V_k,\Gamma_k)\right)\right)\cr
		&g(V_k)\distExp\left(\Gamma_k-\Gamma_{k-1};1\right)
	\]
	This step terminate at $K$ but the hypothetical ``algorithm'' continues. Since $K^\star\le K$, we are conditioning only on $V_k,\Gamma_k$ that have previously been sampled. 
	
	 Our next goal is then to calcualte the probability of the zero set $\Pr\left(x_{1:N,k+1:\infty}=0|\Gamma_k\right)$. One may notice $\{\left(\Gamma,V,x_{1:N}\right)_l\}_{l=k+1}^\infty$ is altogether a Poisson process by a repeated use of marking theorem \cite{kingman92}. Therefore through a simple Poisson counting argument, this probability can be explicitly written as:
	\[
	&\Pr\left(x_{1:N,k+1:\infty}=0|\Gamma_k\right)\cr
	&=\Pr\left(\{\distPP_{(\Gamma,V,x_{1:N})_l}\}_{l=k+1}^\infty\subset\reals\times\reals\times\{(0,0,\cdots,0)\}\right)\cr
	&=\Pr\left(\tN\left(\reals\times\reals\times\ints^+\times\ints^+\times\cdots\times\ints^+\right)=0\right)\cr
	&=\exp\left(-\int\int\sum_{x_{1:N}\ne0}h(x_{1:N}|\tau(v,\gamma))\Lambda_{\Gamma_k}(dv,d\gamma)\right)\cr
	&=e^{-\int_{\reals^2}\left(1-h\left(0|\tau(v,\gamma)\right)^N\right)\Lambda_{\Gamma_k}(dv,d\gamma)}\label{eq:error}
	\]
	where $\Lambda_{\Gamma_k}$ is the rate measure of the marked Poisson process conditional on $\Gamma_k$ and $\tN$ counts the number of points in Poisson process. The rate measure can be calculated by marking theorem, that is for any Borel set $A\in\mcB\left(\reals^2\right)$:
	\[
		\Lambda_{\Gamma_k}\left(A\right)=\int_{(v,\gamma)\in A}g(dv)\ind_{[\Gamma_k,\infty)}\left(d\gamma\right)
	\]
	
	 Equation \ref{eq:error} also bounds L-1 truncation error conditional on $\Gamma_k$ as in \cite{campbell19}. Here we bridge the connection between truncation and slice sampling, that is, if a tight bound of the truncation error exists, then efficient rejection sampling scheme can be developed accordingly. In some cases, it may be convenient to pre-compute the integral and store it in the memory before the iteration starts. One way or the other, one can develop exact sampler for general completely random measures by following this recipe. 
\end{enumerate}

 The algorithm perform above 5 steps in order iteratively. We provide the pseudocode and proof of correctness of this algorithm in the supplementary material. 




==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

